Lecture Notes on Comparison Geometry

This note is based on Professor Vitali Kapovitch's comparison geometry course at the University of Toronto. It delves into various comparison theorems, including those by Rauch and Toponogov, focusing on their applications, such as Bishop-Gromov volume comparison, critical point theory of distance functions, diameter sphere theorem, and negative and nonnegative curvature. Additionally, it covers the soul theorem, splitting theorem, and covering theorem by Cheeger-Gromoll, as well as Perelman's proof of the soul conjecture. Finally, the note introduces Gromov-Hausdorff convergence, Alexandrov Spaces, and the Finite Homotopy type theorem by Grove-Peterson.

==> CH1.tex <==
\chapter*{Introduction to the Comparison Geometry}

==> CH2.tex <==
%%!TEX root = book-template.tex
%book-template
\appendix
\chapter{Review on Riemannian Geometry}
In this appendix, we briefly review the background knowledge on Riemannian geometry that is necessary in this course. 
\section{Riemannian Metric}
A metric $g$ is a smooth covariant $(2, 0)$-tensor field that determines the geometry (length and angle) of a given smooth manifold $M$. At each point $p \in M$, the value $g_p$ is an inner product on $T_pM$. We call a pair $(M, g)$ a Riemannian manifold if $g$ is positive definite at each $p$, i.e. $g_p(v, v) \geq 0$ for each $v \in T_pM$. We use the inner product notation when we want to emphasize the metric $g$ is an inner product at each point:
\begin{equation*}
	\inp{v, w}_g := g_p(v, w), \quad\forall p \in M, v, w \in T_pM.
\end{equation*}
The length of a vector $v$ is denoted as
\begin{equation*}
	\abs{v} := \sqrt{\inp{v, v}_g}
\end{equation*}
If the metric $g$ is understood, we write $\inp{v, w}$ and $\abs{v}$ in the place of $\inp{v, w}_g$ and $\abs{v}_g$. 

The local representations for a metric are important in computations. If $(x^1, \dots, x^n)$ are any local coordinates on an open subset $U \subseteq M$, then $g$ can be locally written, using Einstein summation convention, as 
\begin{equation*}
	g = g_{ij}dx^i\otimes dx^j
\end{equation*}
This allows us to consider $g$ as an $n \times n$-matrix valued function over $M$. At each $p \in M$, the $i,j$-entry of the matrix is evaluated as $g_{ij}(p) = \inp{\partial_i|_p, \partial_j|p}$.

Indeed, one can generalize this representation to any local frame $(E_i)$ and coframe $(\varepsilon^i)$ for $TM$. We can use this representation to determine the orthogonality of a given frame. Namely, a given local frame $(E_i)$ for $M$ on an open set $U$ is said to be orthonormal if $\inp{E_i, E_j} = \delta_{ij}$ in which case $g$ has the local expression $g = \sum_{i = 1}^n \varepsilon^i\otimes\varepsilon^i$.

If $f: (M, g) \to \R$ is smooth, $df_p: T_pM \to \R$ is a linear map. Then by Riesz representation theorem, there is a unique $u \in T_pM$ such that $df_p(v) = \inp{u, v}$ for $v \in T_pM$, we define
	\begin{equation*}
		\grad(f)_p := u
	\end{equation*}
	the gradient vector, then we can define the gradient vector field $\grad(f)$
	
	We can write the gradient in coordinates, that is for $g_{ij}(x) = \inp{\partial_i, \partial_j}$, we have $\grad(f) = g^{ij}\partial_i f\partial_j$. In particular, when the Riemannian manifold is flat then the coordinate vector fields $(\partial_i)$ are orthonormal \cmtv{ this is false.  you also haven't defined flat metrics yet.}. Thus $g_{ij}(p) = \delta_{ij}$ and $\partial_kg_{ij}(p) = 0$, then $\grad(f)_p = \partial_i f\partial_i$. which is a vector field whose components are the same as the component of $df$. We employ the musical isomorphism induced by the Riemannian metric, then we can also write
	\begin{equation*}
		\grad(f) = df^\sharp ;\quad \grad(f)^\flat = df
	\end{equation*}

\begin{definition}[Isometry]\label{def: isometry}
	Let $(M, g), (N, h)$ be Riemannian manifolds with or without boundary. And isometry from $(N, h)$ to $(M, g)$ is a diffeomorphism $\varphi: N \to M$ such that $\varphi^*g = h$, i.e. 
	\begin{equation*}
		h_p(X, Y) = (\varphi^*g)_p(X, Y) := g_{\varphi(p)}(d\varphi_p(X), d\varphi_p(Y))\quad \forall p \in M; X, Y \in T_pM.
	\end{equation*}
	We say $(N, h)$ is isometric to $(M, g)$ if there is an isometry between them. 
\end{definition}
\begin{remark}
	We can always produce an orthonormal frame from a given local frame at each $p \in M$ via the Gram-Schmidt process. However, we will carefully keep in mind that this doesn't mean the local coordinate frames $(\partial_i)$ are orthonormal. This only happens if the metric is flat, i.e. when $g$ is locally isometric to the Euclidean metric.
\end{remark}
\begin{definition}[Induced Riemannian Metric]
	Let $N$ be a differential manifolds and $(M, g)$ be a Riemannian metric, we can induce a metric $h = \varphi^* g$ on $N$ from any immersion $\varphi: N \to M$, i.e.
	\begin{equation*}
		h_p(X, Y) = (\varphi^* g)_p(X, Y) := g_{\varphi(p)}(d\phi_p(X), d\phi_p(X)), \quad\forall p \in M; X, Y \in T_pM
	\end{equation*}
\end{definition}
Comparing this definition with the definition of isometry \ref{def: isometry}, we can easily conclude that any induced Riemannian metric from an immersion is an isometry. \cmtv{ what does that mean?}
\begin{example}
	We can induce a Riemannian metric on a sphere $S^n$ from the Euclidean metric of $\R^{n + 1}$ via the inclusion map $\iota: S^n \to \R^{n + 1}$. The Euclidean metric of $\R^{n + 1}$ is given by 
	\begin{equation*}
		e(x, y) = \inp{x, y} = \sum_{i = 1}^{n + 1}x_iy_i
	\end{equation*}
	It defines a quadratic form \corrv {$Q: \R^n \to \R$,}  then the unit sphere is just the level set 
	\begin{equation*}
		S^n = Q^{-1}(1) = \br{x \in \R^{n + 1}: \inp{x, x} = 1}.
	\end{equation*}
	which is a hypersurface by the regular value theorem, we will show that the inclusion map $\iota$ induces a Riemannian metric. 
	
Indeed, we only need to show $Q(y) > 0$ for any non-zero $y \in T_xS^n$. 
\cmtv{ I don't understand what you are doing here. the level set of a regular value of a function is an embedded submanifold and the metric from the ambient manifold induces a metric on the level set. there is nothing to check for the sphere except checking  that 1 is a regular value of Q.}
A key observation is that 
	\begin{equation*}
		T_xS^n = \br{y \in \R^{n + 1}: \inp{x, y} = 0} = \br{x}^\perp.
	\end{equation*}
	That is because the position vector $x$ is also the normal vector at $x$. Then, for any $y \in T_xS^n$, by the Cauchy-Schwartz, we have
	\begin{equation*}
		\inp{x, x} \inp{y, y} \geq \inp{x, y}^2 \implies Q(y) \geq 0.
	\end{equation*}
	since $\inp{x, x} = 1$ and $\inp{x, y} = 0$. Therefore, the induced metric $g_{S^n} = \iota^* e$ is a Riemannian metric. We call such metric the standard metric of the unit sphere. 

We can induce the Riemannian metric on an $n$-sphere by stereographic projections. Let $S^n$ be an $n$-dimensional sphere, $\mathfrak{N} = (1, 0, \dots, 0)$ and $\mathfrak{S} = (-1, 0, \dots, 0)$ the north and the south poles. Then $\br{U_{\mathfrak{N}}, U_{\mathfrak{S}}}$ is an open cover of $S^n$ where $U_{\mathfrak{N}} = S^n - \br{\mathfrak{N}}$ and $U_{\mathfrak{S}} = S^n - \br{\mathfrak{S}}$. Consider the stereographic projections $\pi_{\mathfrak{N}}: \R^n \to U_{\mathfrak{N}}$ and $\pi_{\mathfrak{S}}: \R^n \to U_{\mathfrak{S}}$, 
	\begin{align*}
		\pi_{\mathfrak{N}}(x_1, x_2, \dots, x_n) = \frac{1}{1 + \abs{x}^2}\brac{\abs{x}^2 - 1, 2x_1, \dots, 2x_n}, \\
		\pi_{\mathfrak{S}}(y_1, y_2, \dots, y_n) = \frac{1}{1 + \abs{y}^2}\brac{1 - \abs{y}^2, 2y_1, \dots, 2y_n}.
	\end{align*}
	where $(x_1, x_2, \dots, x_n), (y_1, y_2, \dots, y_n) \in \R^n$, $\abs{x}^2 = \sum_{i = 1}^n x_i^2$ and $\abs{y}^2 = \sum_{i = 1}^n y_i^2$. We can verify that $\br{(\pi_{\mathfrak{N}}, U_{\mathfrak{N}}), (\pi_{\mathfrak{S}}, U_{\mathfrak{S}})}$ gives a smooth structure on $S^n$. We will denote $g^{\mathfrak{N}}, g^{\mathfrak{S}}$ the Riemannian metrics corresponding to the two parametrizations. Under the parametrization $(U_{\mathfrak{N}}, \pi_{\mathfrak{N}})$ consider $\partial_\alpha \in T_x\R^n \cong \R^n$ where $\alpha = 1, 2, \dots, n$, 
	\begin{align*}
		&d\pi_{\mathfrak{N}}\brac{\partial_\alpha} 
		= \partial_\alpha \pi_{\mathfrak{N}}\\
		&= \brac{\frac{4x_\alpha}{\abs{x}^2 + 1}, \frac{2\delta_{1\alpha}(\abs{x}^2 + 1) - 4x_1x_\alpha}{(\abs{x}^2 + 1)^2}, \dots, \frac{2\delta_{n\alpha}(\abs{x}^2 + 1) - 4x_nx_\alpha}{(\abs{x}^2 + 1)^2}}.
	\end{align*}
 Then we consider the induced metric $e_{\mathfrak{N}} = \pi_{\mathfrak{N}}^*g_{S^n}$ on $\R^n$. Namely,
 \begin{align*}
 	{e_{\mathfrak{N}}}_{\alpha\beta} =& e_{\mathfrak{N}}\brac{\partial_\alpha, \partial_\beta} = g_{S^n}(d\pi_{\mathfrak{N}}\brac{\partial_\alpha}, d\pi_{\mathfrak{N}}\brac{\partial_\beta}) = \inp{\partial_\alpha \pi_{\mathfrak{N}}, \partial_\beta \pi_{\mathfrak{N}}}\\
 	=& \frac{16x_{\alpha\beta}}{(\abs{x}^2 + 1)^4} + \sum_{k = 1}^n\frac{(2\delta_{k\alpha}(\abs{x}^2 + 1) - 4x_k x_\alpha)(2\delta_{k\beta}(\abs{x}^2 + 1) - 4x_k x_\beta)}{(\abs{x}^2 + 1)^4}.\\
 	=& \frac{4\delta_{\alpha\beta}}{(\abs{x}^2 + 1)^2}
 \end{align*}
 Similarly, we have 
 \begin{equation*}
 	{e_{\mathfrak{S}}}_{\alpha\beta} = \frac{4\delta_{\alpha\beta}}{(\abs{y}^2 + 1)^2}
 \end{equation*}
 since $y = \frac{x}{\abs{x}^2}$, then we have on $S^n - \br{\mathfrak{N}, \mathfrak{S}}$, ${e_{\mathfrak{N}}}_{\alpha\beta} = {e_{\mathfrak{S}}}_{\alpha\beta}$. We can conclude that $(\R^n, e_{\mathfrak{N}})$, $(\R^n, e_{\mathfrak{S}})$ and $(S^n, g_{S^n})$ are locally isometric to each other. Indeed, we can say $e_{\mathfrak{N}}$ and $e_{\mathfrak{S}}$ are the local representation of the standard metric $g_{S^n}$ of the sphere. These are useful when we compute the geometric quantities such as volume and curvatures of the sphere. 
 
 We can also use polar coordinates. For simplicity, we consider unit $2$-sphere $S^2$. Consider the polar parameterization $(P, U)$,
 \begin{equation*}
 	P(\theta, \varphi) = (\cos{\theta}, \sin{\theta}\cos{\varphi}, \sin{\theta}\sin{\varphi}).
\end{equation*}
where $(\theta, \varphi) \in U = \br{(\theta, \varphi)| \theta \in (0, \pi), \varphi \in (0, 2\pi)}$. Consider the induced metric on $U$, i.e. $p = P^*g_{S^2}$. Then 
\begin{align*}
	p_{\theta\theta} &= g_{S^2}(\partial_\theta P, \partial_\theta P) = \sin^2{\theta} + \cos^2{\theta}\cos^2{\varphi} + \cos^2{\theta}\sin^2{\varphi} = 1\\
	p_{\theta\varphi} &= g_{S^2}(\partial_\theta P, \partial_\varphi P) = 0\\
	p_{\varphi\varphi} &= g_{S^2}(\partial_\varphi P, \partial_\varphi P) = \sin^2{\theta}d\varphi^2.
\end{align*}
Hence, $p = d\theta^2 + \sin^2{\theta}d\varphi^2$ is a polar local representation of the standard metric $g_{S^n}$.
\end{example}

\begin{example}[Hyperbolic Space]
Indeed, it is also possible to induce a Riemannian metric from an non-Riemannian metric, for example, we can induce a Riemannian metric to hyperbolid from a pseudo-Riemannian metric. Consider a pseudo-Riemannian metric, which is a bilinear form of signature $(n, 1)$ in $\R^{n + 1}$, i.e.
	\begin{equation*}
		\inp{x, y}_{(n, 1)} = \sum_{i = 1}^n x_i\cdot y_i - x_{n + 1}y_{n + 1}
	\end{equation*}
	It defines a unique quadratic form $Q := \inp{\cdot, \cdot}_{n, 1} : \R^{n + 1} \to \R$.\cmtv{ quadratic form has one variable, not two} Then the upper half of the following level set
	\begin{equation*}
		\mathcal{I}^n = Q^{-1}(-1)\cap\br{x_{n + 1} > 0} = \br{x \in \R^{n + 1}: \inp{x, x}_{(n, 1)} = -1, x_{n + 1} > 0}
	\end{equation*}
	is just a hyperboloid which is a hyperspace by regular value theorem, we will show that the the induced metric to $\mathcal{I}^n$ via the inclusion map is a Riemannian metric. We only need to show $Q(y) > 0$ for any non-zero $y \in T_x\mathcal{I}^n$. A key observation is that 
	\begin{equation*}
		T_x\mathcal{I}^n = \br{y \in \R^{n + 1}: \inp{x, y}_{(n, 1)} = 0} = \br{x}^\perp.
	\end{equation*}
	That is because $\mathcal{I}^n$ is a level set of $Q$ so that the gradient of $Q$ is perpendicular to $T_x\mathcal{I}^n$. Let $x = (\hat{x}, x_{n + 1}) \in \mathcal{I}^n$ where $x = (x_1, \dots, x_n)$ and let $0 \neq y = (\hat{y}, y_{n + 1}) \in T_x\mathcal{I}^n$. Clearly if $y_{n + 1} = 0$, then $Q(y) = \hat{y}\cdot\hat{y} > 0$ and we are done. If $y_{n + 1} \neq 0$, then by the observation, we have
	\begin{equation*}
		0 = \inp{x, y}_{(n, 1)} = \hat{x}\cdot\hat{y} - x_{n + 1}y_{n + 1} \iff \hat{x}\cdot\hat{y} = x_{n + 1}y_{n + 1}.
	\end{equation*}
	On the other hand, because $\inp{x, x}_{(n, 1)} = Q(x) = -1$, we know that 
	\begin{equation*}
		\hat{x}\cdot\hat{x} = x_{n + 1}^2 - 1\iff \hat{x}\cdot\hat{x} + 1 = x_{n + 1}^2
	\end{equation*}
	By Cauchy-Schwartz, 
	\begin{align*}
		& (\hat{x}\cdot\hat{x})(\hat{y}\cdot\hat{y})  \geq (\hat{x}\cdot\hat{y})^2 = (x_{n + 1}y_{n + 1})^2 = y_{n + 1}^2(\hat{x}\cdot\hat{x} + 1)\\
		\implies & (\hat{x}\cdot\hat{x})(\hat{y}\cdot\hat{y}) \geq y_{n + 1}^2(\hat{x}\cdot\hat{x}) + y_{n + 1}^2\\
		\iff & (\hat{x}\cdot\hat{x})(\hat{y}\cdot\hat{y} - y_{n + 1}^2) \geq y_{n + 1}^2\\
		\iff & Q(y) = \inp{y, y}_{(n, 1)} \geq \frac{y_{n + 1}^2}{\hat{x}\cdot\hat{x}} > 0
	\end{align*}
	Therefore, denoting the pullback metric by $g_{\mathcal{I}^n}$, we can conclude the $\mathbb{I}^n = (\mathcal{I}^n, g_{\mathcal{I}^n})$ is a Riemannian manifold. 
	
	We can check that, via the stereographic projection $\pi(x) = \frac{\hat{x}}{1 + x_{n + 1}}$ with respect to $(0, \dots, 0, -1)$, $\mathbb{I}^n = (\mathcal{I}^n, g_{\mathcal{I}^n})$ is isometric to $\mathbb{D}^n = (\mathcal{D}^n, g_{\mathcal{D}^n})$ where $\mathcal{D}^n$ is the unit $n$-disk and $g_{\mathcal{D}^n} = \frac{4\sum_{i = 1}^n dx_i^2}{1 - \sum_{i = 1}^n x_i^2}$. 
	
	We can also check that, via $i(x) = 2\frac{x + e_n}{\norm{x + e_n}^2} - e_n$ the inversion with respect to a sphere of center $-e = (0, \dots, 0, -1)$ where $\norm{\cdot}$ is the Euclidean norm on $\R^n$, $g_{\mathcal{I}^n})$ is isometric to $\Pi_+^n = (\pi_+^n, g_{\pi_+^n})$ where $\pi_+^n = \br{x \in \R^n: x > 0}$ and $g_{\pi_+^n} = \frac{\sum_{i = 1}^n dx_i^2}{x_n}$. 
	
	The three Riemannian manifolds $\mathbb{I}^n$, $\mathbb{D}^n$ and $\Pi_+^n$ are all isometric to each other. They are all called hyperbolic space, and in particular, we call $\mathbb{I}^n$ the hyperboloid model, $\mathbb{D}^n$ the Poincare disk model, and $\Pi_+^n$ the upper half space model. 
\end{example}

\section{Connection}
The notion of the connection is motivated from defining ``straight line'' on the curved space.\cmtv{ I don't like this explanation. Connection is motivated by differentiating a vector field. geodesics come from trying to generalize straight lines} In Euclidean space, a curve $\gamma$ is a straight line if and only if we have parametrization for which $\dga'(t) \equiv 0$. The second derivative (acceleration) of the curve being nicely defined in Euclidean space is based on the fact that the Euclidean directional derivative of a vector field in Euclidean space is well defined. However, this is not the case in general. Let $M$ be a manifold embedding in $\R^n$, the Euclidean directional derivative of a tangent vector field is usually non longer the tangent vector field of $M$. An easiest example is to consider a parameterized circle $c(t) = (\cos{\theta}, \sin{\theta})$. The second-order derivative $c''(t)$ is a vector perpendicular to the tangent space. 

 To deal with the issue, we can firstly extend the tangent vector field $Y$ of $M$ to a smooth vector field $\tilde{Y}$ of $\R^n$ and applying the tangential projection $\pi^\top$ after taking the Euclidean derivative.\cmtv{ this doesn't make sense for $\gamma'$} Now, we can define curves that are ``as straight as possible'' to be those curves whose tangential acceleration vanish, i.e. $(\gamma'')^\top := \pi^\top(\gamma''(t)) = 0$. For example, we consider the ``big circle'' of a sphere. \cmtv{ with what parameterization?} Its second order derivative is a vector fields that is perpendicular to the tangent space everywhere along the ``big circle. Thus if we take the tangential projection, the tangential acceleration simply vanishes. In particular, we define this class of curve whose tangential acceleration vanishes as geodesics. 
 
 
By capturing the essential properties of Euclidean and tangential directional derivatives, we can define a way of differentiating sections of vector bundles over manifolds. Let $M$ be a smooth manifold with or without boundary, we denote $\mathfrak{X}(M)$ the space of smooth vector fields over $M$, $\pi: E \to M$ a smooth vector bundle over $M$. And denote $\Gamma(E)$ the space of smooth sections of $E$, we define connection as the rule of doing derivative of smooth sections along vector fields that is independent of the change of coordinates. 
\begin{definition}[Connection]\label{def: connection}
	A \textbf{connection on $E$} is a map
	\begin{equation*}
		\nabla: \mathfrak{X}(M)\times \Gamma(E) \to \Gamma(E)
	\end{equation*}
	written $(X, Y) \to \nabla_XY$, satisfying the following properties:
	\begin{enumerate}
		\item \textbf{Linearity over $C^\infty(M)$ in $X$:} $\forall f_1, f_2 \in C^\infty(M)$ and $X_1, X_2 \in \mathfrak{X}(M)$, and $S \in \Gamma(E)$
			\begin{equation*}
				\nabla_{f_1X_1 + f_2X_2}S = f_1\nabla_{X_1}S + f_2\nabla_{X_2}S.
			\end{equation*}
		\item \textbf{Linearity over $\R$ in $Y$:} $\forall a_1, a_2 \in \R$ and $S_1, S_2 \in \Gamma(M)$, 
			\begin{equation*}
				\nabla_X(a_1S_1 + a_2S_2) = a_1\nabla_XS_1 + a_2\nabla_XS_2
			\end{equation*}
		\item \textbf{Product Rule: } $\forall f \in C^\infty(M)$, $X \in \mathfrak{X}(M)$, $S \in \Gamma(E)$,
			\begin{equation*}
				\nabla_X(fS) = f\nabla_XS + (Xf)S
			\end{equation*}
	\end{enumerate}
	We call the output $\nabla_XY$ the \textbf{covariant derivative of $S$ in the direction $X$}.
\end{definition}
\begin{remark}
	A connection in a smooth section \cmtv{ this sentence is extremely confusing}  in a vector bundle $E$ is linear over $C^\infty(M)$ in $X$	by the property 1.. 
	Thus, given a tangent vector $X_p \in T_pM$ and a smooth section $S$. We can define the directional derivative $\nabla_{X_p}S$. Indeed, we can extend $X_p$ to a smooth vector field $X$ and set $\nabla_{X_p}S = \nabla_XS|_p \in E_p$. One can check that this is well-defined and the directional derivative is independent of the choice of extension.
\end{remark}
\begin{remark}
	Connection is a local operator even if it is defined on global sections. Namely, for $X,\tilde{X} \in \mathfrak{X}(M)$ and $S, \tilde{S} \in \Gamma(E)$, $\nabla_XS|_p = \nabla_{\tilde{X}}\tilde{S}|_p$ if $X = \tilde{X}$ and $S = \tilde{S}$ on a neighborhood of $p$. This neighborhood can be arbitrarily small.
\end{remark}
Now let $\gamma: [a, b] \to M$ a smooth curve such that $\gamma(a) = p$ and $\gamma(b) = q$. 
\begin{definition}[Parallel Section]
	Fix $\nabla$ a connection on $E$, we can define $S$ \textbf{a parallel section along $\gamma$} if $\nabla_{\dot{\gamma}}S = 0$. 
\end{definition}
\begin{proposition}\label{prop: uniqueness of parallel section}
There is a unique parallel section along $\gamma$ under the initial condition $S(a) = v$. 
\end{proposition}
\begin{definition}[Parallel Transport Operator]
	We can define the \textbf{parallel transport operator} $P_\gamma: E_p \to E_q$ taking $P_\gamma(v) = S_v(b)$ for each $v \in E_p$ where $S_v$ is the section with the initial value $v$.  
\end{definition}
\begin{corollary}
	The parallel transport operator $P_{\gamma}: E_p \to E_q$ is a linear isomorphism since it is a linear injective map. Notice that the injectivity of $P_{\gamma}$ follows from the uniqueness Proposition \ref{prop: uniqueness of parallel section}.
\end{corollary}

Next, we define affine connection by restricting our attention to the connection in the tangent bundle $TM$. Remember that $\mathfrak{X}(M) = \Gamma(TM)$ is the space of a smooth vector field on $M$ (smooth section on $TM$).  
\begin{definition}[Affine Connection]
	An \textbf{affine connection} on $M$ is a map 
	\begin{equation*}
		\nabla: \mathfrak{X}(M) \times \mathfrak{X}(M) \to \mathfrak{X}(M)
	\end{equation*}
	satisfying the three properties in the definition of connection \ref{def: connection}. In other words, it is the connection that works especially for smooth vector fields and produces smooth vector fields.
\end{definition}
\begin{definition}[Parallel Vector Field]
	Given an affine connection, we can define $X$ \textbf{a parallel vector field along $\gamma$} if $\nabla_{\dot{\gamma}}X = 0$.
\end{definition}
This definition makes more sense when one wants to define the second-order derivative of a smooth function $f$ on some point $p \in M$. 
\begin{definition}\label{def: 2nd order derivative}
	Let $f \in C^\infty(M)$ and $\nabla$ an affine connection on $M$. Fix $v, w \in T_pM$ for some $p \in M$, we can extend $v, w$ to two smooth vector fields $X, Y$ on $M$. We define \textbf{the second-order derivative of $f$ along $v$ and $w$} as
	\begin{equation*}
		\nabla^2 f(v, w) = [Y(X f) - \nabla_Y X f]|_{p},
	\end{equation*}
	instead of $Y(X f)$, as the latter one depends on the choice of the extension (not well-defined). 
\end{definition}

\begin{proposition}\label{prop: hessian tensor}
	Let $f \in C^\infty(M)$ and $\nabla$ an affine connection on $M$. Then $\nabla^2 f$ is a second-order covariant tensor field on $M$.
	\begin{proof}
		It is sufficient to show that $\nabla^2 f$ admits function linearity with respect to both $X$ and $Y$ entries. The function linearity with respect to $Y$ is trivial. To show $\nabla^2 f$ is function linear with respect to $X$, we consider a smooth function $\phi$, then
		\begin{align*}
			\nabla^2f(\phi X, Y) &= Y(\phi X f)- \nabla_Y(\phi X)f\\
			&= (Y\phi)Xf + \phi Y(X f) - [(Y\phi)X f + \phi\nabla_Y X f]\\
			&= \phi[Y(Xf) - \nabla_Y Xf].
		\end{align*}
	\end{proof}
\end{proposition}

In Euclidean space, the $\nabla^2 f$ is symmetric with respect to $X$ and $Y$ and it is called the Hessian of $f$. However, it is not symmetric for general affine connection on $M$. To make it symmetric we must have 
\begin{equation*}
	X(Yf) - \nabla_X Y f = Y(X f) - \nabla_Y X f
\end{equation*}
which is equivalent to
\begin{equation*}
	(\nabla_X Y - \nabla_Y X - [X, Y])f = 0.
\end{equation*}
\begin{definition}[Torsion]\label{def: torsion}
	Given $\nabla$ an affine connection on $M$, then $\tau(X, Y) := \nabla_X Y - \nabla_Y X - [X, Y]$ defines the \textbf{torsion} of $\nabla$. If $\tau \equiv 0$ on $M$, we say $\nabla$ is \textbf{torsion free}.
\end{definition}

\begin{proposition}\label{prop: torsion tensor}
Given $\nabla$ an affine connection on $M$, $\tau$ is an anti-symmetric tensor. 
\begin{proof}
	for any smooth function $f$, we have
	\begin{align*}
		T(fX, Y) 
		&= \nabla_{fX}Y - \nabla_Y(fX) - [fX, Y]\\
		&= f\nabla_XY - (Yf)X - f\nabla_YX - f[X, Y] + (Yf)X\\
		&= fT(X, Y).
	\end{align*}
\end{proof}
\end{proposition}
\begin{definition}[Symmetric Connection]
	An affine connection $\nabla$ on $M$ is called \textbf{symmetric} if it is torsion-free.
\end{definition}
\begin{definition}[Hessian Operator]
	Let $f$ be a smooth function on $M$, and let $\nabla$ be a symmetric section on $M$. Then for $p \in M$ and any $v, w \in T_pM$, we define $\nabla^2 f(v, w)$ the \textbf{Hessian operator of $f$.}
\end{definition}
\begin{corollary}
	Following our previous discussion, the Hessian operator of $f$ is a symmetric operator.
\end{corollary}



\subsection{Levi-Civita Connection}

Let $\gamma$ be a curve in Euclidean space, then one can easily check that the Euclidean inner product is preserved along two parallel vector fields along $\gamma$, i.e. 
\begin{equation}\label{eq: parallel 0}
	\frac{d}{dt}\inp{X, Y}|_{\gamma} \equiv 0
\end{equation}
for parallel vector fields $X, Y$ along $\gamma$. What if we consider a manifold endowed with a Riemannian metric? The answer is that if we want the equation \ref{eq: parallel 0} to hold in $(M, g)$, we must accept an additional assumption. That is for any $X, Y, Z \in \mathfrak{X}(M)$, we have
\begin{equation}\label{eq: compatible}
	Zg(X, Y) = g(\nabla_Z X, Y) + g(X, \nabla_Z Y).
\end{equation}
\begin{definition}
	The equality \ref{eq: compatible} is called \textbf{compatible condition}. An affine connection $\nabla$ is said to be \textbf{compatible with a Riemannian metric $g$} if the equality \ref{eq: compatible} holds. Given a Riemannian manifold $(M, g)$, a metric connection of $(M, g)$ is the affine connection that is compatible with $g$.  
\end{definition}

Thus, if $\nabla$ is a metric connection on $(M, g)$, for $X, Y$ parallel vector fields along a curve $\sigma$, we have
\begin{equation*}
	\frac{d}{dt}g(X, Y)|_{\gamma} = g(\nabla_{\dot{\gamma}}X, Y) + g(X, \nabla_{\dot{\gamma}}Y) \equiv 0 
\end{equation*}

\begin{definition}[Levi-Civita Connection]
	Let $(M, g)$ be a Riemannian manifold with or without boundary. An affine connection $\nabla$ is said to be a \textbf{Levi-Civita connection} if it is both compatible with $g$ and symmetric. In words, 
	\begin{equation*}
		\br{\text{Levi-Civita connection}} := \br{\text{metric connection}}\cap \br{\text{symmetric connection}}
	\end{equation*}
	\end{definition}
Now we can introduce our famous result in Riemannian geometry. 
\begin{theorem}[Fundamental Theorem of Riemannian Geometry]\label{thm: the fundamental theorem of rm}
	Any Riemannian manifold $(M, g)$ admits a unique Levi-Civita connection.
\end{theorem}


\subsection{Connection in Coordinates}
Using a local frame, we can also express affine connections in coordinates, which is convenient for our computation. Mostly, we consider the local coordinate frame $\br{\partial_i}_{i = 1}^n$ for $TM$ on an open subset $U \subseteq M$. For any indices $i, j \in \br{1, 2, \dots, n}$, we can write $\nabla_{\partial_i}{\partial_j}$ as the linear combination of this frame. Namely,
\begin{equation*}
	\nabla_{\partial_i}\partial_j = \Gamma_{ij}^k\partial_k
\end{equation*}
where $\Gamma_{ij}^k$ is called the \textbf{Christoffel symbol} of $\nabla$ with respect to this coordinate frame. The following proposition gives us an expression of the general vector fields 
\begin{proposition}
	Let $\nabla$ be an affine connection of $M$. For $X, Y \in \mathfrak{X}(U)$, written in terms of the frame as $X = X^i\partial_i$, $Y = Y^j\partial_j$, one has
	\begin{equation*}
		\nabla_XY = \brac{X\brac{Y^k} + X^iY^j\Gamma_{ij}^k}\partial_k.
	\end{equation*}
\end{proposition}
\begin{remark}
	Moreover, one can show that the tangent bundle of each smooth manifold with or without boundary admits a connection and there is a one-to-one correspondence between the connection and the choice of the Christoffel symbols $\br{\Gamma_{ij}^k}$.
\end{remark}
Let $\nabla$ be the Levi-Civita connection on a Riemannian manifold $(M, g)$. Under the local coordinate $\br{x^i}$, 
\begin{equation*}
	g = g_{ij}dx^i\otimes dx^j
\end{equation*}
and the Christoffel symbol under this local coordinate can be expressed as
\begin{equation}\label{eq: Chris in coord}
	\Gamma_{ij}^k = \frac{1}{2}g^{kl}\brac{\partial_{x^i}g_{lj} + \partial_{x^j}g_{li} - \partial_{x^l}g_{ij}}.
\end{equation}

\subsection{Connections on Tensor Bundles}
We can generalize the concept of affine connection from vector fields to tensor fields to define their derivative along a vector field. 
\begin{definition}[Connection on Tensor Bundle]\label{def: connection of tensor bundle}
	Let $F \in \Gamma(T^{(k, l)}TM)$ is an arbitrary smooth section on the tensor bundle $T^{(k, l)}TM$, $\omega^1, \dots, \omega^k$ are smooth $1$-forms and $Y_1, \dots, Y_l$ are smooth vector fields. Then if $\nabla$ is an affine connection on $M$,  we can define the \textbf{connection on the tensor bundle $T^{(k, l)}TM$} as
	\begin{align*}
 	(\nabla_X F)(\omega^1, \dots, \omega^k, Y_1, \dots, Y_l) = X(F(\omega^1, \dots, \omega^k, Y_1, \dots, Y_l))\\
 	- \sum_{i = 1}^kF(\omega^1, \dots, \nabla_X\omega^i ,\dots, \omega^k, Y_1, \dots, Y_l)\\
 	- \sum_{i = 1}^lF(\omega^1, \dots, \omega^k, Y_1, \dots,\nabla_X Y_j , \dots, Y_l)
 \end{align*}
 which is again a $(k, l)$-tensor. We will call $\nabla_X F$ the \textbf{covariant derivative} of $F$ with respect to $X$. And if $\nabla_X F \equiv 0$, then $F$ is said to be \textbf{parallel with respect to $X$.}
\end{definition}
\cmtv{ you have to explain what $\nabla_X\omega$ is}
\begin{corollary}\label{cor: parallel rie metric}
	Any Riemannian metric is parallel with respect to its Levi-Civita connection.  
	\begin{proof}
		This is followed by Definition \ref{def: connection of tensor bundle} and the compatibility condition equation \ref{eq: compatible}.
	\end{proof}
\end{corollary}
\begin{definition}[Total Covariant Derivative]
	Because this covariant derivative $\nabla_X F$ is linear over $C^\infty(M)$ in $X$, we can encode it into a single tensor field $\nabla F$ called the \textbf{total covariant derivative} which is one more than the rank of $F$, as follows
 \begin{equation*}
 	(\nabla F)(\omega^1, \dots, \omega^k, Y_1, \dots, Y_l, X) = (\nabla_X F)(\omega^1, \dots, \omega^k, Y_1, \dots, Y_l)
 \end{equation*}
\end{definition}
\begin{example}
	In particular, for $f: M \to \R$ a smooth function, i.e $f \in \Gamma(T^{(0, 0)}TM)$, and a vector field $X$ on $M$, the total differential is $\nabla f \in \Gamma(T^{(0, 1)}TM)$ such that
 \begin{equation*}
 	(\nabla f)(X) = \nabla_X f = df(X)
 \end{equation*}
 and this is also equal to $g(\grad(f), X)$ if the Riemannian metric $g$ is given. 
\end{example}
\begin{corollary}
We can rewrite Corollary \ref{cor: parallel rie metric} as
	\begin{equation*}
		\nabla g \equiv 0
	\end{equation*}
	if $\nabla$ is the Levi-Civita connection of $g$.
\end{corollary}



\begin{definition}[Second Order Total Covariant Derivative]
Given $X, Y \in \mathfrak{X}(M)$, we can introduce the \textbf{second order total covariant derivative} of a $(k, l)$-tensor field $F$ $\nabla_{X, Y}^2 F$. That is 
 \begin{equation*}
 	\nabla^2_{X, Y}F(\dots) := \nabla^2 F(\dots, Y, X).
 \end{equation*}

\end{definition}
 
  We should be careful that the notation $\nabla^2_{X, Y}F$ is different from $\nabla_X(\nabla_Y F)$ as the latter one is not linear over $C^\infty(M)$ in $Y$. Indeed, one can check that are related as
 \begin{equation}\label{eq: Hessian formula}
 	\nabla^2_{X, Y}F = \nabla_X(\nabla_Y F) - \nabla_{\nabla_X Y}F
 \end{equation}
\begin{definition}
	Let $f \in C^\infty(M)$ then $\nabla^2 f$ is called the covariant Hessian of the operator $u$. By the above formula, we have
 	\begin{align*}
 	\nabla^2f(X, Y) 
 	&= \nabla^2_{Y, X}f = \nabla_Y(\nabla_X f) - \nabla_{\nabla_Y X}f\\
 	&= Y(Xf) - \nabla_YX f
 	\end{align*}
\end{definition}
\begin{remark}
	In particular, when $\nabla$ is symmetric, this definition is consistent with our previous definition of the Hessian operator. 
\end{remark}

\begin{remark}
	Again, if the Riemannian metric is given, we can define the Hessian operator
	\begin{equation*}
		\hess_f = (\nabla^2 f)^\sharp = \nabla((\nabla f)^\sharp) = \nabla(\grad(f))
	\end{equation*}
	Namely, for $X, Y \in \mathfrak{X}(M)$, we have
	\begin{equation*}
		g(\hess_f(X), Y) = \nabla^2 f(X, Y).
	\end{equation*}
\end{remark}


\section{Geodesics, Length, and Distances}
Remember that the notion of covariant derivative is motivated by taking the acceleration of curves on manifolds. Thus, I would like to recall that the above setup allows us to define the covariant derivative of the tensor fields along a curve. That is for any smooth curves $\gamma$, we can induce the covariant derivative $D_t$ such that for any extendible smooth tensor field $F \in C^{\infty}(I; T^{(k, l)}TM)$ along $\gamma$, we have for each $t \in I$
 \begin{equation*}
 	D_t(F(t)) = \nabla_{\gamma'(t)}\tilde{F}
 \end{equation*} 
for any extension $\tilde{F}$, i.e. $F = \tilde{F}\circ\gamma$. Moreover, the operator $D_t$ satisfies the linearity over $\R$ and the product rule over $f \in C^\infty(I)$.



\begin{example}
	In Riemannian geometry, we are particularly interested in the covariant derivative along the tangent vector fields along a given curve. That is $D_t\gamma'$ which is defined as the acceleration of $\gamma$. And $\gamma$ is called a geodesic when 
	\begin{equation*}
		D_t\gamma' \equiv 0
	\end{equation*}
	This is called the geodesic equation. In terms of the local coordinates, we have the local expression of the geodesic equation:
	\begin{equation*}
		x''^k(t) + x'^i(t)x'^j(g)\Gamma_{ij}^k(x(t)) \equiv 0
	\end{equation*}
	Thus we can also say geodesics is the solution of the geodesic equation. And by the existence and uniqueness of the ODE theory, for any $p \in M$, $v \in T_pM$, $t_0 \in \R$, there exists an open interval $t_0 \in I \subseteq \R$ and an unique geodesic $\gamma: I \to M$ such that $\gamma(t_0) = p$ and $\gamma'(t_0) = w$. 
\end{example}

	Given $p \in M$ and $v \in T_pM$, we know there is an unique locally defined geodesic $\gamma$ such that $\gamma(0) = p$ and $\gamma'(0) = v$. Its first-order derivative is
	\begin{equation*}
		(f(\gamma(t)))' = df(\gamma'(t)) = \inp{\grad(f), \gamma'(t)}
	\end{equation*}
	\begin{align*}
		(f(\gamma(t)))'' 
		=& \pd{\inp{\grad(f), \gamma'(t)}}{t} \\
		=& \inp{D_t(\grad(f)), \gamma'(t)} + \inp{\grad(f), \underbrace{D_t(\gamma'(t))}_{\text{$=0$}}}\\
		=&\inp{\nabla_{\gamma'(t)}(\grad(f)), \gamma'(t)}
	\end{align*}
	At $t = 0$ where $\gamma'(0) = v$, we have
	\begin{align*}
		{f(\gamma(t))}''|_{t = 0}
		& = \inp{\nabla_v(\grad (f)), v} = \inp{\nabla(\grad(f))(v), v}\\
		& = \inp{\hess_f(v), v}\\
		& = \nabla^2f(v, v)
	\end{align*}
\begin{remark}
	We have $\nabla^2 f(v, v) = v^T[\frac{\partial^2f}{\partial x_i \partial x_j}]v$ when the metric is flat.
	\cmtv{ as before, this is wrong.}
\end{remark}

We can show that every length-minimizing curve in a Riemannian manifold is a geodesic when it is given a unit-speed parametrization. This is because a length-minimizing curve is a critical point of the length functional. Namely, it certainly satisfies the first variation formula without jump points (we can apply some curve-shortening process to round the corners)
\begin{equation*}
	\dat{s}{0}L_g(\Gamma_s) = -\int_{a}^b\inp{V, D_t\gamma'}dt = 0
\end{equation*}
which in turn solves the geodesic equation when we consider $V = D_t\gamma'$. Conversely, we can say that the geodesic equation characterizes the critical points of the length functional. Therefore, what we indeed concluded is a strengthened corollary such that a unit-speed admissible curve $\gamma$ is a critical point for the length functional $L_g$ if and only if $\gamma$ is a geodesic. 

Be careful that a geodesic is not necessarily length-minimizing. For example, the ``big circle'' on a sphere. However, we know that geodesic is locally minimized. 

We can view $M$ as a metric space, and it is important to discuss whether $M$ is metrically complete. The Hopf-Rinow theory answers this question by characterizing metric completeness by geodesic completeness, i.e. every maximal geodesic is defined for all $t \in \R$. 
	\begin{theorem}[Hopf-Rinow]
		A connected Riemannian manifold is metrically complete if and only if it is geodesically complete.
	\end{theorem}
	We have the following corollaries from the Hopf-Rinow:
	\begin{corollary}
		If $M$ is connected and there is $p \in M$ such that $\exp_p$ is defined on all of $T_pM$, then $M$ is complete. 
	\end{corollary}
	\begin{corollary}
		If $M$ is complete and connected. Then any two points in $M$ can be joined by a minimizing geodesic segment. 
	\end{corollary}
	\begin{corollary}
		If $M$ is complete, then every maximal geodesic in $M$ is defined for all $t\in \R$.
	\end{corollary}
	\section{Curvature Tensor}
	The notion of curvature is motivated from the flatness criterion of Euclidean space. Namely, for vector fields $X, Y, Z \in \mathfrak{X}(\R^n)$, and Euclidean connection $\nabla$, we have
	\begin{equation*}
		\nabla_X\nabla_YZ - \nabla_Y\nabla_XZ = \nabla_{[X, Y]}Z
	\end{equation*}
	An arbitrary connection $\nabla$ on a smooth manifold satisfies flatness criterion if the above equality holds. A Riemannian manifold is called flat if it is locally isometric to Euclidean space.
	\cmtv{ that's not the standard definition. the standard definition is that the curvature is zero.}
	 And we can show that the Levi-Civita connection of a flat Riemannian manifold satisfies the flatness criterion.
	\begin{example}
		An example of flat but not Euclidean Riemannian manifold is a $n$-torus with metric induced by embedding in $\R^{2n}$.\cmtv{ what embedding?}
	\end{example}
	Next, we can define the curvature tensor to be the map $R: \mathfrak{X}(M)\times \mathfrak{X}(M)\times \mathfrak{X}(M) \to \mathfrak{X}(M)$ such that
	\begin{equation*}
		R(X, Y)Z = \nabla_X\nabla_YZ - \nabla_Y\nabla_XZ - \nabla_{[X, Y]}Z
	\end{equation*}
	where $X, Y, Z$ are vector fields on $M$ and $R$ is multilinear over $C^\infty(M)$. Thus this is indeed a $(1, 3)$-tensor fields on $M$. 
	The local representation of $R$ is
	\begin{equation*}
		R = {R_{ijk}}^l dx^i\otimes dx^j\otimes dx^k\otimes \partial_l
	\end{equation*}
	where the coefficient $R_{ijk}^l$ is are defined by $R_{ijk}^l = R(\partial_i, \partial_k)\partial_k$.
	It is more convenient for us to encode the $(1, 3)$-curvature tensor field to be a $(0, 4)$-curvature tensor field by lowering the last index. Namely, we define $Rm = R^\flat$.
	\begin{equation*}
		Rm(X, Y, Z, W) = \inp{R(X, Y)Z, W}
	\end{equation*}
	In terms of the local coordinates, it is written
	\begin{equation*}
		Rm = R_{ijkl}dx^i\otimes dx^j\otimes dx^k\otimes dx^l
	\end{equation*}
	where $R_{ijkl} = g_{lm}{R_{ijk}}^m$. 
	The curvature tensor $Rm$ has symmetries. For all $W, X, Y, Z \in \mathfrak{X}(M)$, we have 
	\begin{itemize}
		\item $Rm(W, X, Y, Z) = -Rm(X, W, Y, Z)$;
		\item $Rm(W, X, Y, Z) = -Rm(W, X, Z, Y)$;
		\item $Rm(W, X, Y, Z) = Rm(Y, Z, W, X)$;
		\item $Rm(W, X, Y, Z) + Rm(X, Y, W, Z) + Rm(Y, W, X, Z) = 0$
	\end{itemize}
	We can think of it as a symmetric map $Rm: \wedge^2M \to \wedge^2M$, so that the first two properties can be viewed as $Rm(W, X, Y, Z) = Rm(W\wedge X, Y\wedge Z)$ a symmetric two linear function. 
	We can define sectional and Ricci curvature, 
	\begin{itemize}
		\item \textbf{Sectional Curvature:} Let $X, Y \in T_pM$ be linearly independent vectors, \begin{equation}
				\sigma = \spa(X, Y)
			\end{equation}
			is a two-subspace in $T_pM$, we can define sectional curvature as
			\begin{equation*}
				\sect(\sigma) := \frac{Rm(X, Y, Y, X)}{\abs{X}^2\abs{Y}^2 - \inp{X, Y}^2}
			\end{equation*}
			The value of $\sect(\sigma)$ is independent from the choice of $X$ and $Y$.
			\begin{proposition}\label{prop: constant sect cur}
				Let $(M, g)$ be a Riemannian manifold, $p \in M$ and $\br{e_1, \dots, e_n}$ an orthonormal basis of $T_pM$. Then $(M, g)$ is a space of constant sectional curvature, i.e. there exists $\kappa_0 \in \R$ such that $\forall p \in M$, $\forall X, Y \in T_pM$, $\sect(\sigma) \equiv \kappa_0$ where $\sigma = \spa(X, Y)$ if and only if
				\begin{equation*}
					R_{ijkl} = \kappa_0(\delta_{ij}\delta_{jk} - \delta_{ik}\delta_{jl}),
				\end{equation*}
				Equivalently, that is $\forall X, Y, Z, W \in \mathfrak{X}(M)$,
				\begin{equation*}
					Rm(X, Y, Z, W) = \kappa_0\brac{\inp{X, Z}\inp{Y, W} - \inp{X, W}\inp{Y, Z}}
				\end{equation*}
			\end{proposition}
			An easier way to compute the sectional curvature is called the moving frame method. Firstly, we can take a standard orthonormal frame $\br{e_1, e_2, \dots, e_3}$ over an open set $U$ of $M$. We define the \textbf{metric $1$-form} $\theta_i \in \Lambda^1(U)$ such that for any $X \in\mathfrak{X}(U)$, 
			\begin{equation*}
				\theta^i(X) = \inp{e_i, X}.
			\end{equation*}
			Therefore, $\theta^i(e_j) = \inp{e_i, e_j} = \delta_{ij}$. Thus, for any $X \in \mathfrak{X}(U)$, 
			\begin{equation*}
				X = \sum_i\theta^i(X)e_i, \quad\inp{X, X} = \sum_i(\theta^i(X))^2
			\end{equation*}
			Therefore, we can rewrite the Riemannian metric as
			\begin{equation*}
				g = \sum_{i}\theta^i\otimes\theta^i
			\end{equation*}
			Furthermore, take
			\begin{equation*}
				\omega_i^j(X) = \inp{\nabla_X e_i, e_j} = \theta^j(\nabla_X e_i) \quad\forall X \in \mathfrak{X}(U)
			\end{equation*}
			Obviously, $\omega_i^j \in \Lambda^1(U)$ and satisfies
			\begin{equation*}
				\nabla_X e_i = \omega_i^j(X)e_j,
			\end{equation*}
			we call $\omega_i^j$ the \textbf{connection form.}
			By the compatibility of the Levi-Civita connection, for any $X \in \mathfrak{X}(U)$, we have
			\begin{align*}
				& \omega_i^j(X) = \inp{\nabla_X e_i, e_j} = X(e_i, e_j) - \inp{e_i, \nabla_X e_j} = -\omega_j^i(X)\\
				\implies & \omega_i^j + \omega_j^i = 0
			\end{align*}
			the connection form is anti-symmetric. 
			Next, we define the \textbf{curvature $2$-form} $\br{R_{ij}}$, for any $X, Y \in \mathfrak{X}(U)$, let
			\begin{equation*}
				R_{ij}(X, Y) := Rm(X, Y, e_i, e_j)
			\end{equation*}
			thus, 
			\begin{equation*}
				R(X, Y)e_i = \sum_{j}R_{ij}(X, Y)e_j
			\end{equation*}
			Denote $\theta = (\theta_1, \theta_2, \dots, \theta_n)^T$, connection matrix $\omega = (\omega_{ij})_{n \times n}$ and the curvature matrix $R = (R_{ij})_{n \times n}$, we can derive the
			\begin{enumerate}
				\item \textbf{The First Cartan Structural Equation: }\begin{equation*}
					d\theta = \omega\wedge \theta.
				\end{equation*}
				Namely, $d\theta_i = -\omega_j^i\wedge\theta^j$.
				\item \textbf{The Second Cartan Structural Equation: }
				\begin{equation*}
					d\omega = \omega\wedge\omega - R.		
				\end{equation*}
				Namely, $d\omega_{ij} = \omega_i^k\wedge\omega_k^j - R_{ij}$. 
			\end{enumerate}
			\begin{theorem}
				There is a unique family ($n^2$-many) of the connection $1$-form $\omega_{ij}$ satisfying
				\begin{equation}\label{eq: connection form system}
					\begin{cases}
						d\theta_i = -\omega_j^i\wedge\theta^j,\\
						\omega_i^j + \omega_j^i = 0.
					\end{cases}
				\end{equation}
			\end{theorem}
			By the above existence and uniqueness theorem, we can first solve the equation system \ref{eq: connection form system} whose solution must be the connection form of the Riemannian manifold, then derive the curvature form by the second Cartan structural equation.
			\begin{example}\label{ex: gauss curvature}
				Consider a $2$-dimensional surface $M$ equipped with the local Riemannian metric $g = \varphi^2 du^2 + \psi^2dv^2$ induced by the local chart $\br{(u, v)}$. Then, then
				\begin{equation*}
					\theta^1 = \varphi du, \quad \theta^2 = \psi dv .
				\end{equation*}
				Then
				\begin{align*}
					d\theta^1 &= d\varphi\wedge du = -\frac{\varphi_v}{\psi}du\wedge\theta^2\\
					d\theta^2 &= d\psi\wedge dv = -\frac{\psi_u}{\varphi}dv\wedge\theta^1
				\end{align*}
				Then we can solve the connection form
				\begin{equation*}
					\omega_1^2 = \frac{\varphi_v}{\psi}du - \frac{\psi_v}{\varphi}dv
				\end{equation*}
				Thus, by the second Cartan equation, we have the curvature form
				\begin{align*}
					R_{12}(e_1, e_2) &= - [(\frac{\psi_v}{\varphi})_u + (\frac{\varphi_v}{\psi})_v]\\
					&= -\frac{1}{\varphi\psi}[(\frac{\psi_v}{\varphi})_u + (\frac{\varphi_v}{\psi})_v]
				\end{align*}
				which is exactly the Gauss curvature.
			\end{example}
			\begin{exercise}
				Let $\kappa > 0$, verify that the Gauss curvature of the rescaled hyperbolic disk, $\mathbb{H}^2 \cong \mathbb{D}_\kappa^2 = (\mathcal{D}_\kappa^2, g_{\mathcal{D}_{\kappa}^2})$ where 
				\begin{align*}
					\mathcal{D}_\kappa^2 &= \br{(x, y) \in \R^2: x^2 + y^2 < \frac{4}{\kappa}}\\
					g_{\mathcal{D}_\kappa^2} &= \frac{dx^2 + dy^2}{(1 - \frac{\kappa}{4}(x^2 + y^2))^2}
				\end{align*}
				is $-\kappa$.
			\end{exercise}
			\begin{example}
				Consider the half-space model of the hyperbolic space $\Pi_+^n = (\pi_+^n, g_{\pi_+^n})$ where 
				\begin{equation*}
					g_{\pi_+^n} = \frac{dx_1^2 + \cdots + dx_n^2}{x_n^2}
				\end{equation*}
				Let $\theta^1 = \frac{dx_1}{x_n}, \dots, \theta^n = \frac{dx_n}{x_n}$, then 
				\begin{align*}
					d\theta^k &= -\frac{1}{x_n^2}dx_n\wedge dx_k = \frac{1}{x_n^2}dx_k\wedge dx_n = \frac{1}{x_n}dx_k\wedge\theta^n \quad k \leq n - 1\\
					d\theta^n &= 0
				\end{align*}
				By the equation system, we can conclude that
				\begin{equation*}
				\begin{cases}
					\omega_i^j = 0, \quad i, j \leq n - 1\\
					\omega_n^k = -\frac{dx_k}{x_n} = -\theta^k \quad k \leq n - 1.
				\end{cases}	
				\end{equation*}
				Next, by the second Cartan structural equation, we have
				\begin{equation*}
				R_{ij} = \omega_i^k\wedge\omega_k^j - d\omega_{ij} = -\theta^i\wedge\theta^j.	
				\end{equation*}
				Therefore for the tangent plane $\sigma = \spa(e_i, e_j)$, the sectional curvature is
				\begin{equation*}
					\sect(\sigma) = R_{ij}(e_i, e_j) = -1.
				\end{equation*}
				In general, for any $i, j, k, l$, we have
				\begin{equation*}
					R_{ijkl} = -(\delta_{ik}\delta_{jl} - \delta_{il}\delta_{jk}).
				\end{equation*}
				Therefore, by the proposition \ref{prop: constant sect cur}, we can conclude that $\Pi_+^n$ is a space of constant curvature $-1$. 
			\end{example}
			
 			\begin{exercise}
 				Consider the rescaled Poincare disk model. Let $\kappa > 0$, $\mathbb{D}^n_\kappa = (\mathcal{D}^n_\kappa, g_{\mathcal{D}^n_\kappa})$ where 
 			\begin{align*}
 				\mathcal{D}^n_\kappa = \br{x \in \R^n: \abs{x}^n < \frac{4}{\kappa}}\\
 				g_{\mathcal{D}^n_\kappa} = \sum_{i = 1}^n\frac{1}{(1 - \frac{\kappa}{4}\abs{x}^2)^2}dx_i^2
 			\end{align*} 
 			We can verify that $D_\kappa^n$ is a space of constant sectional curvature $-\kappa$. 
 			\end{exercise}
		\item \textbf{Ricci Curvature: } If $X_1, \dots, X_n$ is an orthonormal basis of $T_pM$, then we can define we Ricci curvature as the trace of the curvature tensor
			\begin{equation}
				\ric(Y, Z) = \tr(X \mapsto R(X, Y)Z)
			\end{equation}
			Under the orthonormal basis, we can write
			\begin{equation*}
				\ric(Y, Z) = \sum_{i = 1}^n \inp{R(X_i, Y)Z, X_i} = \sum_{i = 1}^n Rm(X_i, Y, Z, X_i)
			\end{equation*} 
			By the previous properties of the curvature tensor
			\begin{equation*}
				Rm(X_i, Y, Z, X_i) = Rm(Z, X_i, X_i, Y) = (-1)(-1)Rm(X_i, Z, Y, X_i)
			\end{equation*}
			therefore, 
			\begin{equation*}
				\ric(Y, Z) = \ric(Z, Y)
			\end{equation*}
	\end{itemize}
	We denote the $n$-dimensional complete simply connected space of constant sectional curvature $\kappa$ by $\modsp{\kappa}$ 
	\begin{itemize}
			\item $\modsp{0} = \R^n$
			\item $\modsp{1} = S_1^n$ a unit sphere.
			\item $\modsp{-1} = \h^n$ the hyperbolic space.
			\item $\modsp{\kappa} = S^n_{\frac{1}{\sqrt{\kappa}}}$ for $\kappa > 0$, the $n$-sphere of radius $\frac{1}{\sqrt{\kappa}}$
			\item $\modsp{\kappa}$ is the hyperbolic space rescaled by factor $\frac{1}{\sqrt{\abs{\kappa}}}$
		\end{itemize}

	\section{Geometry of Riemannian Submanifolds}
	We consider $(M, g)$ a Riemannian submanifold of the ambient Riemannian manifold $(\tilde{M}, \tilde{g})$ where $g = \iota_M^* \tilde{g}$ an induced Riemannian metric by the inclusion map $\iota_M: M \hookrightarrow \tilde{M}$. The submanifold geometry is to study the relation between the geometry of $M$ and of $\tilde{M}$. Our review will mostly follow \cite{Lee19}. 
	
	Let's first compare the Levi-Civita Connection of $M$ and that of $\tilde{M}$. The starting point for doing so is the orthogonal decomposition of the sections of the ambient tangent bundle $T\tilde{M}|_M$ into tangential and orthogonal projection. 
	\begin{notation}
		Denote $\pi^\top: T\tilde{M}|_M \to TM$ the tangential projection and $\pi^\perp: T\tilde{M}|_M \to NM$ the normal projection. \cmtv{ I suggest you use the notation $\nu_M$ instead of $NM$ for the normal bundle as you do elsewhere. }If $X$ is a section of $T\tilde{M}|_M$, we use the shorthand notation $X^\top = \pi^\top X$ and $X^\perp = \pi^\perp X$ for its tangential and normal projection.
	\end{notation}
	\begin{definition}[The Second Fundamental Form (See \cite{Lee19})]
		Let $X, Y \in \mathfrak{X}(M)$, we can extend them to vector fields (still denoted by $X$ and $Y$) on an open subset of $\tilde{M}$. We define \textbf{the second fundamental form of $M$} to be the map $II: \mathfrak{X}(M)\times \mathfrak{X}(M) \to \Gamma(NM)$ given by
		\begin{equation*}
			II(X, Y) = (\tilde{\nabla}_XY)^\perp
		\end{equation*}
	\end{definition}
	Notice that (see proposition 8.1 in \cite{Lee19}), $II(X, Y)$ is bilinear, symmetric, and is independent of the extension of $X, Y \in \mathfrak{X}(M)$ to an open subset of $\tilde{M}$. The value of $II$ at $p$ depends on $X_p$ and $Y_p$. Let $\nabla$ be the Levi-Civita connection on $M$, we have the \textbf{Gauss formula} (see theorem 8.2 in \cite{Lee19}):
	\begin{equation*}
		\tilde{\nabla}_XY = \nabla_XY + II(X, Y).
	\end{equation*}
	The Gauss formula tells us that 
	\begin{equation*}
		\nabla_XY = (\tilde{\nabla}_XY)^\top. 
	\end{equation*}
	If we denote $\nabla^\top_X Y := (\tilde{\nabla}_XY)^\top$, then the connection $\nabla^\top$ induced by $\tilde{\nabla}$ is the unique Levi-Civita connection on $M$, i.e. $\nabla^\top = \nabla$. 
	
	Let $\gamma: I \to M$ be a smooth curve and $X \in \mathfrak{X}(\gamma)$, then we can derive the \textbf{Gauss formula along the curve $\gamma$} (see corollary 8.3 in \cite{Lee19}), i.e.
	\begin{equation*}
		\tilde{D}_tX = D_tX + II(\gamma', X)
	\end{equation*}
	where $\tilde{D}_tX$ and $D_tX$ denotes the covariant derivative along $\gamma$ as a curve in $\tilde{M}$ and as a curve in $M$ respectively. 
	Because $II$ is symmetric and bilinear, we can define a scalar-valued symmetric bilinear form $II_N: \mathfrak{X}(M) \times \mathfrak{X}(M) \to C^\infty(M)$ with respect to each $N \in \Gamma(NM)$ to evaluate the extrinsic covariant derivatives of the normal vector fields. 
	\begin{definition}[Weingarten map in the direction of $N$ (See \cite{Lee19})]
		The scalar-valued symmetric bilinear form $II_N$ induces a self-adjoint operator $W_N: \mathfrak{X}(M) \to \mathfrak{X}(M)$ such that
		\begin{equation*}
			\tilde{g}(W_N(X), Y) = II_N(X, Y) = \inp{N, II(X, Y)}.
		\end{equation*}
		This operator $W_N$ is called the Weingarten map in the direction of $N$.
	\end{definition}
	The Weingarten map evaluates the extrinsic covariant derivative of the normal vector field due to the \textbf{Weingarten Equation} (see proposition 8.4 in \cite{Lee19}  although we use the opposite sign convention than  \cite{Lee19})
	\begin{equation*}
		(\tilde{\nabla}_XN)^\top = W_N(X) \quad \forall X \in \mathfrak{X}(M)
	\end{equation*}
	and any $N \in \Gamma(NM)$ extended arbitrarily to an open subset of $\tilde{M}$.
	
	By the \textbf{Gauss equation} (see theorem 8.5 in \cite{Lee19}), for all $W, X, Y, Z \in \mathfrak{X}(M)$,
	\begin{equation*}
		\tilde{Rm}(W, X, Y, Z) = \tilde{Rm}(W, X, Y, Z) - \inp{II(W, Z), II(X, Y)} + \inp{II(W, Y), II(X, Z)}.
	\end{equation*}
	which means that the second fundamental form also describes the difference between the curvature tensors of $\tilde{M}$ and $M$.
	
	Another fundamental equation for submanifolds is called the \textbf{Codazzi equation}. That is for all $W, X, Y \in \mathfrak{X}(M)$, we have
	\begin{equation*}
		(\tilde{R}(W, X)Y)^\perp = (\nabla_W^F II)(X, Y) - (\nabla_W^F II)(W, Y).
	\end{equation*}
	Recall that $F \to M$ is the bundle whose fiber at each $p \in M$ is the set of bilinear maps $T_pM \times T_pM \to N_pM$. And $\nabla^F$ is a connection defined by
	\begin{equation*}
		(\nabla_X^F B)(X, Y) = \nabla_X^\perp(B(Y, Z)) - B(\nabla_XY, Z) - B(Y, \nabla_XZ).
	\end{equation*}
	where $B$ can be any smooth section of $F$. For example, the second fundamental form $II$. The sign $\nabla^\perp: \mathfrak{X}(M) \times \Gamma(NM) \to \Gamma(NM)$ is the normal connection defined by
	\begin{equation*}
		\nabla_X^\perp N = (\tilde{\nabla}_X N)^\perp
	\end{equation*}
	Because $(N_1, (\tilde{\nabla}_X N_2)^\top) = 0$, for any two sections $N_1, N_2 \in \Gamma(NM)$ and $X \in \mathfrak{X}(M)$, we have
	\begin{align*}
		X\tilde{g}(N_1, N_2) 
		&= \tilde{g}(\tilde{\nabla}_X N_1, N_2) + (N_1, \tilde{\nabla}_X N_2)\\
		&= \tilde{g}((\tilde{\nabla}_X N_1)^\perp, N_2) + \tilde{g}(N_1, (\tilde{\nabla}_X N_2)^\perp)\\
		&= \tilde{g}(\tilde{\nabla}^\perp_X N_1, N_2) + \tilde{g}(N_1, \tilde{\nabla}^\perp_X N_2)
	\end{align*}
	Therefore, the normal section is also compatible with $\tilde{g}$. 
	
	Let $\gamma: I \to M$ be a unit speed curve. Then we can define the intrinsic curvature of $\gamma$ as
	\begin{equation*}
		\kappa(t) = \abs{D_t\gamma'(t)}.
	\end{equation*}
	If we consider $\gamma$ as a curve in $\tilde{M}$, we can also define the extrinsic curvature $\tilde{\kappa}$ as
	\begin{equation*}
		\tilde{\kappa}(t) = \abs{\tilde{D}_t\gamma'(t)}
	\end{equation*}
	Then geometrically (see proposition 8.10 in \cite{Lee19}), for any $p \in M$ and $v \in T_pM$, $II(v, v)$ is the $\tilde{g}$-acceleration at $p$ of the $g$-geodesic $\gamma_v$ and $|II(v, v)|$ is the $\tilde{g}$-curvature of $\gamma_v$ at $p$. Indeed the second fundamental form is completely determined by its value of the form $II(v, v)$ for unit vectors $v$ by lemma 8.11 in \cite{Lee19}.
	\begin{definition}[Totally geodesic]
		A Riemannian submanifold $(M, g)$ of $(\tilde{M}, \tilde{g})$ is said to be totally geodesic if the second fundamental form of $M$ vanishes identically.
	\end{definition}
	By proposition 8.12 in \cite{Lee19}, the geometric interpretation of totally geodesic is that every $\tilde{g}$ geodesic that is tangent to $M$ at some $t_0$ stays in $M$ for all $t$ in some interval $(t_0 - \epsilon, t_0 + \epsilon)$. Equivalently, this also means every $g$-geodesic in $M$ is also $\tilde{g}$-geodesic in $\tilde{M}$.
	
	In this note, we are particularly interested in the case when $M$ is a hypersurface in $\tilde{M}$. Because the codimension is $1$, there are only two consistent choices of the unit normal vector field in a small neighborhood. Thus, we can fix $N$ locally and rewrite the scalar second fundamental form $h^N = II_N$ (If we pick $-N$, we will have the corresponding $-h^N$). Also, we will use the notation $S^N = W_N$ and call it the \textbf{shape operator of $M$}. 
	From our previous discussion on the scalar second fundamental form and the Weingarten map, we have the following corollaries about the connections on the hypersurface, $h^N$ and $S^N$
\begin{itemize}
    \item $h^N$ is a symmetric and bilinear form, i.e. for all $X, Y \in \mathfrak{X}(M)$ and $f \in C^\infty(M)$,
	\begin{equation*}
    	f h^N(X, Y) = f h^N(Y, X) = h^N(fX, Y) = h^N(X, fY).
    \end{equation*}
    \item $S^N$ is self-adjoint, i.e. for all $X, Y \in \mathfrak{X}(M)$,\begin{equation*}
    	\tilde{g}(S^N(X), Y) = \tilde{g}(S^N(Y), X).
    \end{equation*}
    \item $\nabla^\perp_X N$ is tangent to the hypersurface $M$, that is because \begin{equation*}
    	X\tilde{g}(N, N) = 2\tilde{g}(\nabla^\perp_X N, N) = 0.
    \end{equation*}
    \item For $X, Y \in \mathfrak{X}(M)$, if we extend $X, Y$ to an open subset of $\tilde{M}$ and assume $[X, Y] = 0$, as a Levi-Civita connection, we have $\tilde{\nabla}_X Y = \tilde{\nabla}_Y X$, then 
    \begin{align*}
    	&0 = X\tilde{g}(N, Y) = \tilde{g}(\nabla^\perp_X N, Y) + \tilde{g}(\nabla^\perp_X Y, N)\\
    	&0 = Y\tilde{g}(N, X) = \tilde{g}(\nabla^\perp_Y N, X) + \tilde{g}(\nabla^\perp_Y X, N)\\
    	\implies &  \tilde{g}(\nabla^\perp_Y N, X) = -\tilde{g}(\nabla^\perp_X N, Y)
    \end{align*}
\end{itemize}	
	We introduce the notation \textbf{Kulkarni-Nomizu product} of symmetric $2$-tensors $h, k$ is
	\begin{equation*}
		h\owedge k(w, x, y, z) = h(w, z)k(x, y) + h(x, y)k(x, z) - h(w, y)k(x, z) - h(x, z)k(w, y)
	\end{equation*}\
	and the \textbf{exterior covariant derivative} of a symmetric $2$-tensor field $T$ 
	\begin{equation*}
		(DT)(x, y, z) = -(\nabla T)(x, y, z) + (\nabla T)(x, z, y).
	\end{equation*}
	so that we are able to rewrite the previous formulas and equations more simply in the case of a hypersurface (see theorem 8.13 in \cite{Lee19}). 
	\begin{itemize}
		\item \textbf{Gauss Formula for a Hypersurface}: For $X, Y \in\mathfrak{X}(M)$ vector fields extended to an open subset of $\tilde{M}$\begin{equation}
			\tilde{\nabla}_XY = \nabla_XY + h^N(X, Y)N.
		\end{equation}
		\item \textbf{Gauss Formula for a Curve in a Hypersurface}: Let $\gamma: I \to M$ be a smooth curve and $X: I \to TM \in \mathfrak{X}(\gamma)$, \begin{equation}
			\tilde{D}_tX = D_tX + h^N(\gamma', X)N.
		\end{equation}
		\item \textbf{Weingarten Equation for a Hypersurface}: For $X \in \mathfrak{X}(M)$,\begin{equation}\label{eq: weingarten for hyper}
			\tilde{\nabla}_XN = S^N(X).
		\end{equation}
		\item \textbf{Gauss Equation for a Hypersurface}: For all $W, X, Y, Z \in \mathfrak{X}(M)$, \begin{equation}
			\tilde{Rm}(W, X, Y, Z) = Rm(W, X, Y, Z) - \frac{1}{2}(h^N\owedge h^N)(W, X, Y, Z).
		\end{equation}
		\item \textbf{Codazzi Equation for a Hypersurface}: For all $W, X, Y \in \mathfrak{X}(M)$, \begin{equation}
			\tilde{Rm}(W, X, Y, N) = (Dh^N)(Y, W, X).
		\end{equation}
	\end{itemize}
	
	
	
	
	

==> notations.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{dnf}[theorem]{Definitions and Facts}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{question}[theorem]{Question}
\newtheorem{property}[theorem]{Property}
\newtheorem{properties}[theorem]{Properties}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{note}[theorem]{Notes}
\newtheorem{conj}[theorem]{Conjecture}

\newcommand{\cut}{\mathbf{Cut}}
\newcommand{\mres}{\mathbin{\vrule height 1.6ex depth 0pt width
0.13ex\vrule height 0.13ex depth 0pt width 1.3ex}}
\newcommand{\dga}{\dot{\gamma}}
\newcommand{\ddga}{\ddot{\gamma}}
\newcommand{\dddga}{\dddot{\gamma}}
\newcommand{\sss}{\sum_{i=1}^{n}}
\newcommand{\nvec}{\Vec{\mathbf{n}}}
\newcommand{\tvec}{\Vec{\mathbf{t}}}
\newcommand{\bvec}{\Vec{\mathbf{b}}}
\newcommand{\nvecs}{\Vec{\mathbf{n}}_s}
\newcommand{\tvecs}{\Vec{\mathbf{t}}_s}
\newcommand{\bvecs}{\Vec{\mathbf{b}}_s}
\newcommand{\arccur}{\gamma(s)}
\newcommand{\ds}[1]{\frac{d#1}{ds}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diff}[2]{\frac{d #1}{d #2}}
\newcommand{\ddiff}[2]{\frac{d^2 #1}{{d #2}^2}}
\newcommand{\sgn}{\mathbf{sgn}}

\newcommand{\unfinished}{\textcolor{green}{Haven’t finished}}
\newcommand{\emb}{\mathbf{Emb}}
\newcommand{\re}{\mathfrak{Re}}
\newcommand{\im}{\mathfrak{Im}}
\newcommand{\spn}{\mathbf{span}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\RP}{\mathbb{RP}}
%\newcommand{\kk}{G}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Om}{\Omega}
\newcommand{\Si}{\Sigma}
\newcommand{\G}{\Gamma}
\newcommand{\M}{\textbf{M}}
\newcommand{\haus}{\mathcal{H}}
%\newcommand{\diam}{\textbf{diam}}
\DeclareMathOperator{\diam}{\textbf{diam}}
\DeclareMathOperator{\rad}{\textbf{rad}}

\newcommand{\supp}{\mathbf{supp}\,}

\newcommand{\ind}{\mathbf{index}}
\newcommand{\br}[1]{\left\{#1\right\}}
\newcommand{\inp}[1]{\langle #1 \rangle}
\newcommand{\brac}[1]{\left(#1\right)}
\newcommand{\rms}[1]{\mathcal{M}^{k}} %space of C^k riemannian metrics
\newcommand{\edge}{\mathscr{E}} %edges
\newcommand{\vertex}{\mathscr{V}} %vertices
\newcommand{\eprod}[2]{\langle #1, #2\rangle}
\newcommand{\length}{\mathbf{Length}}
\newcommand{\grad}{\mathbf{grad}}
\newcommand{\id}{\mathbf{Id}}
\newcommand{\dive}{\mathbf{div}}
\newcommand{\hess}{\mathbf{Hess}}
\newcommand{\ric}{\mathbf{Ric}}
\newcommand{\sect}{\mathbf{Sec}}
\newcommand{\scal}{\mathbf{Scal}}
\newcommand{\tr}{\mathbf{Trace}}
\renewcommand{\det}[1]{\mathbf{det}{(#1)}}
\newcommand{\vol}{\mathbf{Vol}}
\newcommand{\dist}{\mathbf{dist}}
\newcommand{\graph}{\mathbf{graph}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\dat}[2]{\frac{d}{d{#1}}\Bigr|_{{#1} = {#2}}}
\newcommand{\ddat}[2]{\frac{d^2}{d{#1}^2}\Bigr|_{{#1} = {#2}}}

\newcommand{\pik}{\varpi^\kappa}


%\newcommand{\Zk}{Z_l(M, \partial M; \mathbb{Z}_2)}
\newcommand{\Zk}{Z_k(M, \partial M; G)}
\newcommand{\Ztworel}{Z_2(\Omega, \partial \Omega; \mathbb{Z}_2)}
\newcommand{\Ztwo}{Z_2(\Omega; \mathbb{Z}_2)}
\newcommand{\F}{\mathcal{F}}
\newcommand{\eps}{\varepsilon}
\newcommand{\modsp}[1]{\mathbb{M}_{#1}^n}
\newcommand{\mdk}{\mathbf{md}_\kappa}
\newcommand{\snk}{\mathbf{sn}_\kappa}
\newcommand{\csk}{\mathbf{cs}_\kappa}
\newcommand{\cs}{\mathbf{cs}}
\newcommand{\ctk}{\mathbf{ct}_\kappa}

\newcommand{\tnk}{\mathbf{tan}_\kappa}
\newcommand{\an}{An}
\newcommand{\ans}{\mathcal{AN}}


\providecommand{\abs}[1]{\lvert #1\rvert}
\providecommand{\norm}[1]{\lvert\lvert #1\rvert\rvert}


\newcommand{\qst}[1]{\textcolor{red}{(\textbf{Question: }{#1})}}
\newcommand{\cmt}[1]{\textcolor{blue}{(\textbf{Comments: }{#1})}}
\newcommand{\cmtv}[1]{\textcolor{magenta}{(\textbf{Vitali: }{#1})}}
\newcommand{\xinze}[1]{\textcolor{orange}{(\textbf{Xinze: }{#1})}}

\newcommand{\corrv}[1]{\textcolor{ForestGreen}{{#1}}}


\newcommand{\op}{\mathbf{Op}}
\newcommand{\sing}{\mathbf{sing}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\fo}{\mathscr{F}}
\newcommand{\splm}{\mathcal{L}}
\newcommand{\spdo}{\mathbf{Diff}}
\newcommand{\sh}{\mathfrak{Sh}}
\newcommand{\inj}{\mathbf{Injrad}}

\newcommand{\ghto}{\xrightarrow{\mathbf{G-H}}}

\newcommand{\pghto}{\xrightarrow{\text{pointed $\mathbf{G-H}$}}}
\newcommand{\spa}{\mathbf{Span}}
\newcommand{\radg}{\mathfrak{R}}
\newcommand{\modangle}{\Tilde{\measuredangle}}
\newcommand{\modtriangle}{\Tilde{\triangle}}
\newcommand{\mtr}[3]{[\Tilde{#1}\Tilde{#2}\Tilde{#3}]}
\newcommand{\modcvee}{\Tilde{\curlyvee}}
\newcommand{\mangle}{\measuredangle}
\newcommand{\peri}{\mathbf{Per}}
\newcommand{\acts}{\curvearrowright}
\newcommand{\rank}{\mathbf{rank}}
\newcommand{\h}{\mathbb{H}}
\newcommand{\alex}{\mathfrak{Alex}}


\newcommand{\sn}{\mathbf{sn}}
\newcommand{\md}{\mathbf{md}}
\newcommand{\modspace}[1]{\mathbb{M}^2\brac{#1}}
\def\dashint{\,\ThisStyle{\ensurestackMath{%
  \stackinset{c}{.2\LMpt}{c}{.5\LMpt}{\SavedStyle-}{\SavedStyle\phantom{\int}}}%
  \setbox0=\hbox{$\SavedStyle\int\,$}\kern-\wd0}\int}
\newcommand{\bigzero}{\mbox{\normalfont\Large\bfseries 0}}
\newcommand{\rvline}{\hspace*{-\arraycolsep}\vline\hspace*{-\arraycolsep}}
\newcommand{\isom}{\textbf{Isom}}

\newcommand{\CR}{\mathfrak{CompRad}}
\newcommand{\curv}{curv}

\newcommand{\aut}{\mathbf{Aut}}

